Stochastic Binning and Coded Demixing for Unsourced Random Access

Unsourced random access is a novel communication paradigm designed for handling a large number of uncoordinated users that sporadically transmit very short messages. Under this model, coded compressed sensing (CCS) has emerged as a low-complexity scheme that exhibits good error performance. Yet, one of the challenges faced by CCS pertains to disentangling a large number of codewords present on a single factor graph. To mitigate this issue, this article introduces a modified CCS scheme whereby active devices stochastically partition themselves into groups that utilize separate sampling matrices with low cross-coherence for message transmission. At the receiver, ideas from the field of compressed demixing are employed for support recovery, and separate factor graphs are created for message disambiguation in each cluster. This reduces the number of active users on a factor graph, which improves performance significantly in typical scenarios. Indeed, coded demixing reduces the probability of error as the number of groups increases, up to a point. Findings are supported with numerical simulations.

==> other.tex <==
\appendices

\section{Estimator}

For the sake of exposition, suppose that the estimator only has access to the portion of the effective observation that pertains to its own bin.
Then, under the asymptotic AMP characterization, the probability density of a specific section assignment is given by
\begin{equation*}
\begin{split}
&
\begin{split}
f(\rv_b (\ell), \mathcal{S}_b)
&= \binom{K}{K_b} \frac{(B - 1)^{K - K_b}}{B^{K}} \prod_{i \notin \mathcal{S}_b} f \left( \frac{\rv_b(\ell, i)}{\tau} \right) \\
&\qquad \times \prod_{j \in \mathcal{S}_b} f \left( \frac{\rv_b(\ell, j) - d}{\tau} \right)
\end{split} \\
% &= \binom{K}{K_b} \left(1 - \frac{1}{B} \right)^K \prod_{i} f \left( \frac{\rv_b(\ell, i)}{\tau} \right) \\
% &\qquad \times \frac{1}{(B-1)^{K_b}} \prod_{j \in \mathcal{S}_b} \exp \left( \frac{d \rv_b(\ell, j)}{\tau^2} - \frac{d^2}{2 \tau^2} \right) \\
&= \binom{K}{K_b} \left( 1 - \frac{1}{B} \right)^K \prod_{i} f \left( \frac{\rv_b(\ell, i)}{\tau} \right) \\
&\qquad \times \frac{1}{(B-1)^{K_b}}
\exp \left( \frac{d \sum_{j \in \mathcal{S}_b} (2\rv_b(\ell,j) - d)}{2 \tau^2} \right)
\end{split}
\end{equation*}
where $f(\cdot)$ denotes the density of a standard Gaussian random variable, $\mathcal{N}(0,1)$.

\begin{equation*}
\begin{split}
&f(\rv_b (\ell), K_b)
= \sum_{\mathcal{S}_b : |\mathcal{S}_b|=K_b} f(\rv_b (\ell), \mathcal{S}_b) \\
&= \binom{K}{K_b} \left( 1 - \frac{1}{B} \right)^K \prod_{i} f \left( \frac{\rv_b(\ell, i)}{\tau} \right) \\
&\times \frac{1}{(B-1)^{K_b}} \sum_{\mathcal{S}_b : |\mathcal{S}_b|=K_b}
\exp \left( \frac{d \sum_{j \in \mathcal{S}_b} (2\rv_b(\ell,j) - d)}{2 \tau^2} \right)
\end{split}
\end{equation*}




Suppose that one only has access to information from 
Under , the statistic
\begin{equation*}
r_b = \left\langle \rv_b, \mathbf{1} \right\rangle = \textstyle \sum_{\ell, \kappa} \rv_b (\ell, \kappa)
\end{equation*}
is approximately Gaussian with conditional distribution $\mathcal{N} (d L K_b, m L \tau_t^2)$ given $K_b$.
Likewise, the statistic
\begin{equation*}
r_{!b} = \textstyle \sum_{b' \neq b} \left\langle \rv_{b'}, \mathbf{1} \right\rangle
= \left\langle \rv, \mathbf{1} \right\rangle - r_b,
\end{equation*}
conditioned on $K_b$, is approximately Gaussian with density $\mathcal{N} \left( d L (\Ktot - K_b), m L (B-1) \tau_t^2 \right)$.
In addition, these two random variables become conditionally independent for a large system.
Based on the above characterization, we can derive a minimum mean square error (MMSE) estimator for $K_b$ that takes as input $r_b$ and $r_{!b}$,
\begin{equation*}
\begin{split}
&\hat{K}_b (r_b, r_{!b}) = \mathrm{E} \left[ K_b | R_b = r_b, R_{!b} = r_{!b} \right] \\
&= \textstyle \sum_{K_b=0}^K K_b \binom{K}{K_b} \frac{(B - 1)^{K - K_b}}{B^{K}}
\frac{f_{R_b, R_{!b} | K_b} (r_b, r_{!b})}{f_{R_b, R_{!b}} (r_b, r_{!b})} .
\end{split}
\end{equation*}

\begin{align*}
R_b &\sim \mathcal{N} (d L K_b, m L \tau_t^2) \\
R_{!b} &\sim \mathcal{N} \left( d L (K - K_b), m L (B-1) \tau_t^2 \right) \\
\end{align*}
The conditional distribution for observation pair $(R_b, R_{!b})$, given $K_b$, can be expressed as
\begin{equation} \label{equation:PairConditionalDistribution}
\begin{split}
f_{R_b, R_{!b} | K_b} (r_b, r_{!b})
&= \frac{1}{2 \pi \sigma_b \sigma_{!b}} \exp \left( - \frac{(r_b - d L K_b)^2}{2  m L \tau_t^2} \right) \\
&\times \exp \left( - \frac{(r_{!b} - d L (K - K_b))^2}{2 m L (B-1) \tau_t^2} \right) .
\end{split}
\end{equation}
This immediately leads to unconditioned density
\begin{equation} \label{equation:PairDistribution}
f_{R_b, R_{!b}} (r_b, r_{!b})
= \sum_{K_b = 0}^K f_{R_b, R_{!b} | K_b} (r_b, r_{!b}) \Pr (K_b) .
\end{equation}


The minimum mean square error (MMSE) estimator for this system is given explicitly by the standard form
\begin{equation*}
\begin{split}
&\hat{K}_b (r_b, r_{!b}) = \mathrm{E} \left[ K_b | R_b = r_b, R_{!b} = r_{!b} \right] \\
&= \sum_{K_b=0}^K K_b \Pr (K_b | R_b = r_b, R_{!b} = r_{!b}) \\
&= \sum_{K_b=0}^K K_b \frac{f_{R_b, R_{!b} | K_b} (r_b, r_{!b}) \Pr (K_b)}{f_{R_b, R_{!b}} (r_b, r_{!b})} \\
&= \sum_{K_b=0}^K K_b \binom{K}{K_b} \frac{(B - 1)^{K - K_b}}{B^{K}}
\frac{f_{R_b, R_{!b} | K_b} (r_b, r_{!b})}{f_{R_b, R_{!b}} (r_b, r_{!b})}
\end{split}
\end{equation*}

\begin{figure}[t]
\centerline{
\input{Figures/PUPE_with_Estimators}}
\caption{PUPE with Estimation. }
  \label{fig:pupe_results}
\end{figure}




\begin{equation*}
\begin{split}
&
\begin{split}
f(\rv_b (\ell); \varepsilon)
&= \sum_{K_b = 0}^m
\sum_{\mathcal{S}_b : |\mathcal{S}_b| = K_b} \varepsilon^{K_b} (1 - \varepsilon)^{m - K_b} \\
&\qquad \times \prod_{i \notin \mathcal{S}_b} f \left( \frac{\rv_b(\ell, i)}{\tau} \right)
\prod_{j \in \mathcal{S}_b} f \left( \frac{\rv_b(\ell, j) - d}{\tau} \right)
\end{split} \\
&= \prod_{i} \left( (1 - \varepsilon) f \left( \frac{\rv_b(\ell, i)}{\tau} \right)
+ \varepsilon f \left( \frac{\rv_b(\ell, i) - d}{\tau} \right) \right) \\
&= \prod_{i} f \left( \frac{\rv_b(\ell, i)}{\tau} \right)
\prod_{j} \left( 1 - \varepsilon
+ \varepsilon \exp \left( \frac{ d \rv_b(\ell,j)}{\tau^2} - \frac{d^2}{2 \tau^2} \right) \right)
\end{split}
\end{equation*}

\begin{equation*}
\begin{split}
&\operatorname*{arg\,max}_{\epsilon} \log \prod_{\ell} f(\rv_b (\ell); \varepsilon) \\
&= \operatorname*{arg\,max}_{\epsilon} \sum_{j, \ell} \log \left( 1 - \varepsilon
+ \varepsilon \exp \left( \frac{ d \rv_b(\ell,j)}{\tau^2} - \frac{d^2}{2 \tau^2} \right) \right)
\end{split}
\end{equation*}

\begin{equation*}
\sum_{j,\ell} \frac{\exp \left( \frac{ d \rv_b(\ell,j)}{\tau^2} - \frac{d^2}{2 \tau^2} \right) - 1}{1
+ \varepsilon \left( \exp \left( \frac{ d \rv_b(\ell,j)}{\tau^2} - \frac{d^2}{2 \tau^2} \right) - 1 \right)}
\end{equation*}


